Counting Colored Tilings on Grids and Graphs

In this paper, we explore some generalizations of a counting problem related to tilings in grids of size 2xn, which was originally posed as a question on Mathematics Stack Exchange (Question 3972905). In particular, we consider this problem for the product of two graphs G and P(n), where P(n) is the path graph of n vertices. We give explicit bivariate generating functions for some specific cases.

==> eptcsdata.tex <==
\providecommand{\firstpage}{164}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2024\\
EPTCS 403, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.403.33}{10.4204/EPTCS.403.33}}

